Measurement of the $CP$ asymmetry in $B^-\to D_s^-D^0$ and $B^-\to D^-D^0$ decays

The $CP$ asymmetry in $B^-\to D_s^-D^0$ and $B^-\to D^-D^0$ decays is measured using LHCb data corresponding to an integrated luminosity of 3.0 fb$^{-1}$, collected in $pp$ collisions at centre-of-mass energies of 7 and 8 TeV. The results are $A^{CP}(B^-\to D_s^-D^0)=(-0.4\pm 0.5\pm 0.5)\%$ and $A^{CP}(B^-\to D^-D^0)=( 2.3\pm 2.7\pm 0.4)\%$, where the first uncertainties are statistical and the second systematic. This is the first measurement of $A^{CP}(B^-\to D_s^-D^0)$ and the most precise determination of $A^{CP}(B^-\to D^-D^0)$. Neither result shows evidence of $CP$ violation.

==> LHCb_Authorship_flat_arXiv_20-Feb-2018.tex <==
LHCb collaboration: 
R. Aaij,
B. Adeva,
M. Adinolfi,
Z. Ajaltouni,
S. Akar,
P. Albicocco,
J. Albrecht,
F. Alessio,
M. Alexander,
A. Alfonso Albero,
S. Ali,
G. Alkhazov,
P. Alvarez Cartelle,
A.A. Alves Jr,
S. Amato,
S. Amerio,
Y. Amhis,
L. An,
L. Anderlini,
G. Andreassi,
M. Andreotti,
J.E. Andrews,
R.B. Appleby,
F. Archilli,
P. d'Argent,
J. Arnau Romeu,
A. Artamonov,
M. Artuso,
E. Aslanides,
M. Atzeni,
G. Auriemma,
S. Bachmann,
J.J. Back,
S. Baker,
V. Balagura,
W. Baldini,
A. Baranov,
R.J. Barlow,
S. Barsuk,
W. Barter,
F. Baryshnikov,
V. Batozskaya,
V. Battista,
A. Bay,
J. Beddow,
F. Bedeschi,
I. Bediaga,
A. Beiter,
L.J. Bel,
N. Beliy,
V. Bellee,
N. Belloli,
K. Belous,
I. Belyaev,
E. Ben-Haim,
G. Bencivenni,
S. Benson,
S. Beranek,
A. Berezhnoy,
R. Bernet,
D. Berninghoff,
E. Bertholet,
A. Bertolin,
C. Betancourt,
F. Betti,
M.O. Bettler,
M. van Beuzekom,
Ia. Bezshyiko,
S. Bifani,
P. Billoir,
A. Birnkraut,
A. Bizzeti,
M. Bj{\o}rn,
T. Blake,
F. Blanc,
S. Blusk,
V. Bocci,
O. Boente Garcia,
T. Boettcher,
A. Bondar,
N. Bondar,
S. Borghi,
M. Borisyak,
M. Borsato,
F. Bossu,
M. Boubdir,
T.J.V. Bowcock,
E. Bowen,
C. Bozzi,
S. Braun,
M. Brodski,
J. Brodzicka,
D. Brundu,
E. Buchanan,
C. Burr,
A. Bursche,
J. Buytaert,
W. Byczynski,
S. Cadeddu,
H. Cai,
R. Calabrese,
R. Calladine,
M. Calvi,
M. Calvo Gomez,
A. Camboni,
P. Campana,
D.H. Campora Perez,
L. Capriotti,
A. Carbone,
G. Carboni,
R. Cardinale,
A. Cardini,
P. Carniti,
L. Carson,
K. Carvalho Akiba,
G. Casse,
L. Cassina,
M. Cattaneo,
G. Cavallero,
R. Cenci,
D. Chamont,
M.G. Chapman,
M. Charles,
Ph. Charpentier,
G. Chatzikonstantinidis,
M. Chefdeville,
S. Chen,
S.-G. Chitic,
V. Chobanova,
M. Chrzaszcz,
A. Chubykin,
P. Ciambrone,
X. Cid Vidal,
G. Ciezarek,
P.E.L. Clarke,
M. Clemencic,
H.V. Cliff,
J. Closier,
V. Coco,
J. Cogan,
E. Cogneras,
V. Cogoni,
L. Cojocariu,
P. Collins,
T. Colombo,
A. Comerma-Montells,
A. Contu,
G. Coombs,
S. Coquereau,
G. Corti,
M. Corvo,
C.M. Costa Sobral,
B. Couturier,
G.A. Cowan,
D.C. Craik,
A. Crocombe,
M. Cruz Torres,
R. Currie,
C. D'Ambrosio,
F. Da Cunha Marinho,
C.L. Da Silva,
E. Dall'Occo,
J. Dalseno,
A. Danilina,
A. Davis,
O. De Aguiar Francisco,
K. De Bruyn,
S. De Capua,
M. De Cian,
J.M. De Miranda,
L. De Paula,
M. De Serio,
P. De Simone,
C.T. Dean,
D. Decamp,
L. Del Buono,
B. Delaney,
H.-P. Dembinski,
M. Demmer,
A. Dendek,
D. Derkach,
O. Deschamps,
F. Dettori,
B. Dey,
A. Di Canto,
P. Di Nezza,
S. Didenko,
H. Dijkstra,
F. Dordei,
M. Dorigo,
A. Dosil Su{\'a}rez,
L. Douglas,
A. Dovbnya,
K. Dreimanis,
L. Dufour,
G. Dujany,
P. Durante,
J.M. Durham,
D. Dutta,
R. Dzhelyadin,
M. Dziewiecki,
A. Dziurda,
A. Dzyuba,
S. Easo,
U. Egede,
V. Egorychev,
S. Eidelman,
S. Eisenhardt,
U. Eitschberger,
R. Ekelhof,
L. Eklund,
S. Ely,
A. Ene,
S. Escher,
S. Esen,
H.M. Evans,
T. Evans,
A. Falabella,
N. Farley,
S. Farry,
D. Fazzini,
L. Federici,
G. Fernandez,
P. Fernandez Declara,
A. Fernandez Prieto,
F. Ferrari,
L. Ferreira Lopes,
F. Ferreira Rodrigues,
M. Ferro-Luzzi,
S. Filippov,
R.A. Fini,
M. Fiorini,
M. Firlej,
C. Fitzpatrick,
T. Fiutowski,
F. Fleuret,
M. Fontana,
F. Fontanelli,
R. Forty,
V. Franco Lima,
M. Frank,
C. Frei,
J. Fu,
W. Funk,
C. F{\"a}rber,
E. Gabriel,
A. Gallas Torreira,
D. Galli,
S. Gallorini,
S. Gambetta,
M. Gandelman,
P. Gandini,
Y. Gao,
L.M. Garcia Martin,
B. Garcia Plana,
J. Garc{\'\i}a Pardi{\~n}as,
J. Garra Tico,
L. Garrido,
D. Gascon,
C. Gaspar,
L. Gavardi,
G. Gazzoni,
D. Gerick,
E. Gersabeck,
M. Gersabeck,
T. Gershon,
Ph. Ghez,
S. Gian{\`\i},
V. Gibson,
O.G. Girard,
L. Giubega,
K. Gizdov,
V.V. Gligorov,
D. Golubkov,
A. Golutvin,
A. Gomes,
I.V. Gorelov,
C. Gotti,
E. Govorkova,
J.P. Grabowski,
R. Graciani Diaz,
L.A. Granado Cardoso,
E. Graug{\'e}s,
E. Graverini,
G. Graziani,
A. Grecu,
R. Greim,
P. Griffith,
L. Grillo,
L. Gruber,
B.R. Gruberg Cazon,
O. Gr{\"u}nberg,
E. Gushchin,
Yu. Guz,
T. Gys,
C. G{\"o}bel,
T. Hadavizadeh,
C. Hadjivasiliou,
G. Haefeli,
C. Haen,
S.C. Haines,
B. Hamilton,
X. Han,
T.H. Hancock,
S. Hansmann-Menzemer,
N. Harnew,
S.T. Harnew,
C. Hasse,
M. Hatch,
J. He,
M. Hecker,
K. Heinicke,
A. Heister,
K. Hennessy,
L. Henry,
E. van Herwijnen,
M. He{\ss},
A. Hicheur,
D. Hill,
P.H. Hopchev,
W. Hu,
W. Huang,
Z.C. Huard,
W. Hulsbergen,
T. Humair,
M. Hushchyn,
D. Hutchcroft,
P. Ibis,
M. Idzik,
P. Ilten,
K. Ivshin,
R. Jacobsson,
J. Jalocha,
E. Jans,
A. Jawahery,
F. Jiang,
M. John,
D. Johnson,
C.R. Jones,
C. Joram,
B. Jost,
N. Jurik,
S. Kandybei,
M. Karacson,
J.M. Kariuki,
S. Karodia,
N. Kazeev,
M. Kecke,
F. Keizer,
M. Kelsey,
M. Kenzie,
T. Ketel,
E. Khairullin,
B. Khanji,
C. Khurewathanakul,
K.E. Kim,
T. Kirn,
S. Klaver,
K. Klimaszewski,
T. Klimkovich,
S. Koliiev,
M. Kolpin,
R. Kopecna,
P. Koppenburg,
S. Kotriakhova,
M. Kozeiha,
L. Kravchuk,
M. Kreps,
F. Kress,
P. Krokovny,
W. Krupa,
W. Krzemien,
W. Kucewicz,
M. Kucharczyk,
V. Kudryavtsev,
A.K. Kuonen,
T. Kvaratskheliya,
D. Lacarrere,
G. Lafferty,
A. Lai,
G. Lanfranchi,
C. Langenbruch,
T. Latham,
C. Lazzeroni,
R. Le Gac,
A. Leflat,
J. Lefran{\c{c}}ois,
R. Lef{\`e}vre,
F. Lemaitre,
P. Lenisa,
O. Leroy,
T. Lesiak,
B. Leverington,
P.-R. Li,
T. Li,
Z. Li,
X. Liang,
T. Likhomanenko,
R. Lindner,
F. Lionetto,
V. Lisovskyi,
X. Liu,
D. Loh,
A. Loi,
I. Longstaff,
J.H. Lopes,
D. Lucchesi,
M. Lucio Martinez,
A. Lupato,
E. Luppi,
O. Lupton,
A. Lusiani,
X. Lyu,
F. Machefert,
F. Maciuc,
V. Macko,
P. Mackowiak,
S. Maddrell-Mander,
O. Maev,
K. Maguire,
D. Maisuzenko,
M.W. Majewski,
S. Malde,
B. Malecki,
A. Malinin,
T. Maltsev,
G. Manca,
G. Mancinelli,
D. Marangotto,
J. Maratas,
J.F. Marchand,
U. Marconi,
C. Marin Benito,
M. Marinangeli,
P. Marino,
J. Marks,
G. Martellotti,
M. Martin,
M. Martinelli,
D. Martinez Santos,
F. Martinez Vidal,
A. Massafferri,
R. Matev,
A. Mathad,
Z. Mathe,
C. Matteuzzi,
A. Mauri,
E. Maurice,
B. Maurin,
A. Mazurov,
M. McCann,
A. McNab,
R. McNulty,
J.V. Mead,
B. Meadows,
C. Meaux,
F. Meier,
N. Meinert,
D. Melnychuk,
M. Merk,
A. Merli,
E. Michielin,
D.A. Milanes,
E. Millard,
M.-N. Minard,
L. Minzoni,
D.S. Mitzel,
A. Mogini,
J. Molina Rodriguez,
T. Momb{\"a}cher,
I.A. Monroy,
S. Monteil,
M. Morandin,
G. Morello,
M.J. Morello,
O. Morgunova,
J. Moron,
A.B. Morris,
R. Mountain,
F. Muheim,
M. Mulder,
D. M{\"u}ller,
J. M{\"u}ller,
K. M{\"u}ller,
V. M{\"u}ller,
P. Naik,
T. Nakada,
R. Nandakumar,
A. Nandi,
I. Nasteva,
M. Needham,
N. Neri,
S. Neubert,
N. Neufeld,
M. Neuner,
T.D. Nguyen,
C. Nguyen-Mau,
S. Nieswand,
R. Niet,
N. Nikitin,
A. Nogay,
D.P. O'Hanlon,
A. Oblakowska-Mucha,
V. Obraztsov,
S. Ogilvy,
R. Oldeman,
C.J.G. Onderwater,
A. Ossowska,
J.M. Otalora Goicochea,
P. Owen,
A. Oyanguren,
P.R. Pais,
A. Palano,
M. Palutan,
G. Panshin,
A. Papanestis,
M. Pappagallo,
L.L. Pappalardo,
W. Parker,
C. Parkes,
G. Passaleva,
A. Pastore,
M. Patel,
C. Patrignani,
A. Pearce,
A. Pellegrino,
G. Penso,
M. Pepe Altarelli,
S. Perazzini,
D. Pereima,
P. Perret,
L. Pescatore,
K. Petridis,
A. Petrolini,
A. Petrov,
M. Petruzzo,
B. Pietrzyk,
G. Pietrzyk,
M. Pikies,
D. Pinci,
F. Pisani,
A. Pistone,
A. Piucci,
V. Placinta,
S. Playfer,
M. Plo Casasus,
F. Polci,
M. Poli Lener,
A. Poluektov,
N. Polukhina,
I. Polyakov,
E. Polycarpo,
G.J. Pomery,
S. Ponce,
A. Popov,
D. Popov,
S. Poslavskii,
C. Potterat,
E. Price,
J. Prisciandaro,
C. Prouve,
V. Pugatch,
A. Puig Navarro,
H. Pullen,
G. Punzi,
W. Qian,
J. Qin,
R. Quagliani,
B. Quintana,
B. Rachwal,
J.H. Rademacker,
M. Rama,
M. Ramos Pernas,
M.S. Rangel,
F. Ratnikov,
G. Raven,
M. Ravonel Salzgeber,
M. Reboud,
F. Redi,
S. Reichert,
A.C. dos Reis,
C. Remon Alepuz,
V. Renaudin,
S. Ricciardi,
S. Richards,
K. Rinnert,
P. Robbe,
A. Robert,
A.B. Rodrigues,
E. Rodrigues,
J.A. Rodriguez Lopez,
A. Rogozhnikov,
S. Roiser,
A. Rollings,
V. Romanovskiy,
A. Romero Vidal,
M. Rotondo,
M.S. Rudolph,
T. Ruf,
J. Ruiz Vidal,
J.J. Saborido Silva,
N. Sagidova,
B. Saitta,
V. Salustino Guimaraes,
C. Sanchez Mayordomo,
B. Sanmartin Sedes,
R. Santacesaria,
C. Santamarina Rios,
M. Santimaria,
E. Santovetti,
G. Sarpis,
A. Sarti,
C. Satriano,
A. Satta,
D. Savrina,
S. Schael,
M. Schellenberg,
M. Schiller,
H. Schindler,
M. Schmelling,
T. Schmelzer,
B. Schmidt,
O. Schneider,
A. Schopper,
H.F. Schreiner,
M. Schubiger,
M.H. Schune,
R. Schwemmer,
B. Sciascia,
A. Sciubba,
A. Semennikov,
E.S. Sepulveda,
A. Sergi,
N. Serra,
J. Serrano,
L. Sestini,
P. Seyfert,
M. Shapkin,
Y. Shcheglov,
T. Shears,
L. Shekhtman,
V. Shevchenko,
B.G. Siddi,
R. Silva Coutinho,
L. Silva de Oliveira,
G. Simi,
S. Simone,
N. Skidmore,
T. Skwarnicki,
I.T. Smith,
M. Smith,
l. Soares Lavra,
M.D. Sokoloff,
F.J.P. Soler,
B. Souza De Paula,
B. Spaan,
P. Spradlin,
F. Stagni,
M. Stahl,
S. Stahl,
P. Stefko,
S. Stefkova,
O. Steinkamp,
S. Stemmle,
O. Stenyakin,
M. Stepanova,
H. Stevens,
S. Stone,
B. Storaci,
S. Stracka,
M.E. Stramaglia,
M. Straticiuc,
U. Straumann,
S. Strokov,
J. Sun,
L. Sun,
K. Swientek,
V. Syropoulos,
T. Szumlak,
M. Szymanski,
S. T'Jampens,
Z. Tang,
A. Tayduganov,
T. Tekampe,
G. Tellarini,
F. Teubert,
E. Thomas,
J. van Tilburg,
M.J. Tilley,
V. Tisserand,
M. Tobin,
S. Tolk,
L. Tomassetti,
D. Tonelli,
R. Tourinho Jadallah Aoude,
E. Tournefier,
M. Traill,
M.T. Tran,
M. Tresch,
A. Trisovic,
A. Tsaregorodtsev,
A. Tully,
N. Tuning,
A. Ukleja,
A. Usachov,
A. Ustyuzhanin,
U. Uwer,
C. Vacca,
A. Vagner,
V. Vagnoni,
A. Valassi,
S. Valat,
G. Valenti,
R. Vazquez Gomez,
P. Vazquez Regueiro,
S. Vecchi,
M. van Veghel,
J.J. Velthuis,
M. Veltri,
G. Veneziano,
A. Venkateswaran,
T.A. Verlage,
M. Vernet,
M. Vesterinen,
J.V. Viana Barbosa,
D.  Vieira,
M. Vieites Diaz,
H. Viemann,
X. Vilasis-Cardona,
A. Vitkovskiy,
M. Vitti,
V. Volkov,
A. Vollhardt,
B. Voneki,
A. Vorobyev,
V. Vorobyev,
C. Vo{\ss},
J.A. de Vries,
C. V{\'a}zquez Sierra,
R. Waldi,
J. Walsh,
J. Wang,
M. Wang,
Y. Wang,
Z. Wang,
D.R. Ward,
H.M. Wark,
N.K. Watson,
D. Websdale,
A. Weiden,
C. Weisser,
M. Whitehead,
J. Wicht,
G. Wilkinson,
M. Wilkinson,
M.R.J. Williams,
M. Williams,
T. Williams,
F.F. Wilson,
J. Wimberley,
M. Winn,
J. Wishahi,
W. Wislicki,
M. Witek,
G. Wormser,
S.A. Wotton,
K. Wyllie,
D. Xiao,
Y. Xie,
A. Xu,
M. Xu,
Q. Xu,
Z. Xu,
Z. Xu,
Z. Yang,
Z. Yang,
Y. Yao,
H. Yin,
J. Yu,
X. Yuan,
O. Yushchenko,
K.A. Zarebski,
M. Zavertyaev,
L. Zhang,
Y. Zhang,
A. Zhelezov,
Y. Zheng,
X. Zhu,
V. Zhukov,
J.B. Zonneveld,
S. Zucchelli

==> Makefile <==
# $Id: Makefile 87305 2016-02-08 13:50:32Z lafferty $
# ===============================================================================
# Purpose: simple Makefile to streamline processing latex document (just say "make" to execute)
# Author: Tomasz Skwarnicki
# Created on: 2010-09-24
# A few changes by Patrick Koppenburg on 2015-06-26
# ===============================================================================

# name of the main latex file (do not include .tex)
MAIN = main

# name of the target - change that to something descriptive, like paper-v0, Bs2PhiPhi-ANA-v1, etc...
TARGET = template

# name of command to perform Latex (either pdflatex or latex)
LATEX = pdflatex

ifeq ($(LATEX),pdflatex)
	FIGEXT = .pdf
	MAINEXT= .pdf
	BUILDCOMMAND=rm -f $(MAIN).aux && $(LATEX) $(MAIN) && bibtex $(MAIN) && $(LATEX) $(MAIN) && $(LATEX) $(MAIN)
	BUILDCOMMANDPRL=rm -f $(MAIN)-prl.aux && $(LATEX) $(MAIN)-prl && bibtex $(MAIN)-prl && $(LATEX) $(MAIN)-prl && $(LATEX) $(MAIN)-prl
	MAKEMAINCOUNT= sed 's\#{wordcount}{false}\#{wordcount}{true}\#' main-prl.tex > main-count.tex
	BUILDCOMMANDCOUNT= $(MAKEMAINCOUNT) && rm -f $(MAIN)-count.aux && $(LATEX) $(MAIN)-count && bibtex $(MAIN)-count >/dev/null; true && $(LATEX) $(MAIN)-count && ./wordcount.sh $(MAIN)-count && rm wordcount.pdf main-count* 
else
	FIGEXT = .eps
	MAINEXT= .pdf
	BUILDCOMMAND=rm -f $(MAIN).aux && $(LATEX) $(MAIN) && bibtex $(MAIN) && $(LATEX) $(MAIN) && $(LATEX) $(MAIN) && dvips -z -o $(MAIN).ps $(MAIN) && ps2pdf $(MAIN).ps && rm -f head.tmp body.tmp
	BUILDCOMMANDPRL=rm -f $(MAIN)-prl.aux && $(LATEX) $(MAIN)-prl && bibtex $(MAIN)-prl && $(LATEX) $(MAIN)-prl && $(LATEX) $(MAIN)-prl && dvips -z -o $(MAIN)-prl.ps $(MAIN)-prl && ps2pdf $(MAIN)-prl.ps && rm -f head.tmp body.tmp
	BUILDCOMMANDCOUNT=
endif

# list of all source files
TEXSOURCES = $(wildcard *.tex) $(wildcard *.bib)
FIGSOURCES = $(wildcard figs/*$(FIGEXT))
SOURCES    = $(TEXSOURCES) $(FIGSOURCES)

# define output (could be making .ps instead)
OUTPUT = $(TARGET)$(MAINEXT)

# cp temporary main.pdf to target.
$(OUTPUT): $(MAIN)$(MAINEXT)
	cp $(MAIN)$(MAINEXT) $(OUTPUT)

# prescription how to make output (your favorite commands to process latex)
# do latex twice to make sure that all cross-references are updated 
$(MAIN)$(MAINEXT): $(SOURCES) Makefile
	$(BUILDCOMMAND)

# just so we can say "make all" without knowing the output name
all: $(OUTPUT)

# remove temporary files (good idea to say "make clean" before putting things back into repository)
.PHONY : clean
clean:
	rm -f *~ *.aux *.log *.bbl *.blg *.dvi *.tmp *.out *.blg *.bbl $(OUTPUT) $(MAIN)$(MAINEXT) $(MAIN).ps $(MAIN)-prl.ps $(MAIN)-prlNotes.bib

# remove output file
rmout: 
	rm $(OUTPUT) $(MAIN)$(MAINEXT)

# Make the PRL version
prl: 
	$(BUILDCOMMANDPRL)

# Make the PRL version
count: 
	$(BUILDCOMMANDCOUNT)
	@echo ''
	@echo 'Figures:   Add 20+150/(aspect ratio) per figure'
	@echo 'Equations: Add 16 words per row (single column) '
	@echo 'Tables:    Add 13 words plus 6.5 words per line (single column)'
	@echo 

